Neural Media Bias Detection Using Distant Supervision With BABE -- Bias Annotations By Experts

Media coverage has a substantial effect on the public perception of events. Nevertheless, media outlets are often biased. One way to bias news articles is by altering the word choice. The automatic identification of bias by word choice is challenging, primarily due to the lack of a gold standard data set and high context dependencies. This paper presents BABE, a robust and diverse data set created by trained experts, for media bias research. We also analyze why expert labeling is essential within this domain. Our data set offers better annotation quality and higher inter-annotator agreement than existing work. It consists of 3,700 sentences balanced among topics and outlets, containing media bias labels on the word and sentence level. Based on our data, we also introduce a way to detect bias-inducing sentences in news articles automatically. Our best performing BERT-based model is pre-trained on a larger corpus consisting of distant labels. Fine-tuning and evaluating the model on our proposed supervised data set, we achieve a macro F1-score of 0.804, outperforming existing methods.

==> take_out.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ABSTRACT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Media coverage possesses a substantial effect on the public perception of events. Nevertheless, nearly all media outlets are known to report news in a biased way. . One of the ways in which bias in news articles can be introduced is by altering word choice. To identify bias by word choice automatically is a difficult task, especially due to the a lack of a large-scale gold-standard data set and high context-dependencies. In this paper, we present a prototypical yet robust and diverse data set, created by trained expert annotators, for media bias research. We also analyze why expert labeling should be favored within this domain. Our data set outperforms existing work in data quality, while also reaching an inter-annotator agreement of .5 measured by Krippendorff's $\alpha$. It consists of 3700 sentences balanced among topics and news outlets and contains labels for media bias on the word and sentence level. Based on our data, we also introduce a way to detect bias-inducing sentences in news articles automatically. Our neural model uses bias-specific BERT embeddings and is considering information on sentence level bias when optimizing the loss function. Our approach achieves an accuracy of 76.80\% and a F1-score of 70.61, outperforming currently available methods.
